Constraint-Conditioned Policy Optimization for Versatile Safe Reinforcement Learning

Safe reinforcement learning (RL) focuses on training reward-maximizing agents subject to pre-defined safety constraints. Yet, learning versatile safe policies that can adapt to varying safety constraint requirements during deployment without retraining remains a largely unexplored and challenging area. In this work, we formulate the versatile safe RL problem and consider two primary requirements: training efficiency and zero-shot adaptation capability. To address them, we introduce the Conditioned Constrained Policy Optimization (CCPO) framework, consisting of two key modules: (1) Versatile Value Estimation (VVE) for approximating value functions under unseen threshold conditions, and (2) Conditioned Variational Inference (CVI) for encoding arbitrary constraint thresholds during policy optimization. Our extensive experiments demonstrate that CCPO outperforms the baselines in terms of safety and task performance while preserving zero-shot adaptation capabilities to different constraint thresholds data-efficiently. This makes our approach suitable for real-world dynamic applications.

==> Tables/ablation_new.tex <==
\begin{table}[H]
% \begin{wrapfigure}{R}{0.6\textwidth}
% \begin{minipage}{0.7\textwidth}
  \centering
  \vspace{-10pt}
\caption{\small 
Ablation study of removing the versatile value function estimation (VVE), and the conditioned variational inference (CVI). $\uparrow$: the higher reward, the better. $\downarrow$: the lower constraint violation (minimal 0), the better. Each value is reported as mean ± standard deviation for 50 episodes and 5 seeds.
% Evaluation results of natural performance (no attack), under MC and MR attackers, and the average of them. 
Each value is reported as mean ± standard deviation. 
% Failure agents are marked with $\star$.
}
\scriptsize
    \begin{tabular}{ccccccc}
    \toprule
    Algorithm & Stats & Ball-Circle & Car-Circle & Drone-Circle & Drone-Run & Ant-Run \\
    \midrule
    \multirow{4}[2]{*}{CCPO (Full)} & Avg. R $\uparrow$ & \cellcolor[rgb]{ .906,  .902,  .902}710.86\tiny{±20.47} & \cellcolor[rgb]{ .906,  .902,  .902}406.06\tiny{±6.30} & \cellcolor[rgb]{ .906,  .902,  .902}630.55\tiny{±40.03} & \cellcolor[rgb]{ .906,  .902,  .902}458.69\tiny{±12.98} & \cellcolor[rgb]{ .906,  .902,  .902}660.88\tiny{±4.82} \\
          & Avg. CV $\downarrow$ & \cellcolor[rgb]{ .906,  .902,  .902}0.59\tiny{±0.31} & \cellcolor[rgb]{ .906,  .902,  .902}1.60\tiny{±0.91} & \cellcolor[rgb]{ .906,  .902,  .902}0.32\tiny{±0.38} & \cellcolor[rgb]{ .906,  .902,  .902}0.23\tiny{±0.25} & \cellcolor[rgb]{ .906,  .902,  .902}3.13\tiny{±1.67} \\
          & Avg. R-G $\uparrow$ & \cellcolor[rgb]{ .906,  .902,  .902}699.04\tiny{±20.48} & \cellcolor[rgb]{ .906,  .902,  .902}401.53\tiny{±5.59} & \cellcolor[rgb]{ .906,  .902,  .902}625.51\tiny{±40.12} & \cellcolor[rgb]{ .906,  .902,  .902}455.64\tiny{±11.83} & \cellcolor[rgb]{ .906,  .902,  .902}660.07\tiny{±5.26} \\
          & Avg. CV-G $\downarrow$ & \cellcolor[rgb]{ .906,  .902,  .902}0.83\tiny{±0.42} & \cellcolor[rgb]{ .906,  .902,  .902}1.49\tiny{±0.38} & \cellcolor[rgb]{ .906,  .902,  .902}0.47\tiny{±0.55} & \cellcolor[rgb]{ .906,  .902,  .902}0.33\tiny{±0.37} & \cellcolor[rgb]{ .906,  .902,  .902}3.25\tiny{±1.48} \\
    \midrule
    \multirow{4}[2]{*}{CCPO w/o VVE} & Avg. R $\uparrow$ & 674.55\tiny{±17.81} & 370.42\tiny{±14.38} & 426.47\tiny{±49.30} & 417.84\tiny{±8.24} & 428.59\tiny{±88.39} \\
          & Avg. CV $\downarrow$ & 0.60\tiny{±0.41} & 6.42\tiny{±0.85} & 8.67\tiny{±1.45} & 3.28\tiny{±2.86} & 10.66\tiny{±11.81} \\
          & Avg. R-G $\uparrow$ & 670.61\tiny{±14.18} & 364.5\tiny{±14.51} & 416.83\tiny{±47.46} & 413.28\tiny{±9.04} & 434.59\tiny{±83.89} \\
          & Avg. CV-G $\downarrow$ & 0.93\tiny{±0.36} & 5.64\tiny{±0.92} & 7.74\tiny{±1.36} & 3.33\tiny{±3.16} & 12.01\tiny{±10.08} \\
    \midrule
    \multirow{4}[2]{*}{CCPO w/o CVI} & Avg. R $\uparrow$ & 641.33\tiny{±40.14} & 387.31\tiny{±5.76} & 520.70\tiny{±42.18} & 386.81\tiny{±39.44} & 465.80\tiny{±31.78} \\
          & Avg. CV $\downarrow$ & 1.44\tiny{±0.72} & 1.66\tiny{±0.79} & 2.36\tiny{±2.67} & 0.81\tiny{±0.76} & 3.51\tiny{±0.93} \\
          & Avg. R-G $\uparrow$ & 623.17\tiny{±41.42} & 383.24\tiny{±6.30} & 519.05\tiny{±36.31} & 388.69\tiny{±35.35} & 465.36\tiny{±32.20} \\
          & Avg. CV-G $\downarrow$ & 1.78\tiny{±0.70} & 2.17\tiny{±1.09} & 2.73\tiny{±3.03} & 1.15\tiny{±1.08} & 3.96\tiny{±1.01} \\
    \bottomrule
    \end{tabular}%
  % \label{tab:ablation}%
  \vspace{-10pt}
% \end{minipage}
% \end{wrapfigure}
\end{table}%



==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerYes{} See Conclusion section.
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerYes{} See Conclusion section.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerYes{}
        \item Did you include complete proofs of all theoretical results?
   % \answerYes{} See Appendix \ref{app:proof}.
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerYes{} See supplementary material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    % \answerYes{} See Appendix \ref{app:implementation}.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    % \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerYes{} See Appendix \ref{app:implementation}.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    % \answerYes{}
  \item Did you mention the license of the assets?
    % \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    % \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    % \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    % \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    % \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    % \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    % \answerNA{}
\end{enumerate}


\end{enumerate}

==> misc.tex <==
We use $\overline{\mathcal{S}} \times \overline{\mathcal{A}}$ to denote the set of state-action pairs that are forbidden by some constraint.

\section{Scope}
Training robustness. Adversarial exist during training and testing.

Testing robustness. Adversarial only exist during testing.

\section{Observational Adversarial Attacker for Safe RL}
What is the goal of the attacker in safe RL? 
It is not like a robust adversarial RL setting, which is a zero-sum game, where the attacker's objective is simply minimizing the rewards.
In safe RL, since safety constraints are incorporated, the objective for the attacker may not be that obvious.
The goals could be:
\begin{enumerate}
    \item Only maximizing constraint violations.
    \item Only minimizing rewards.
    \item Maximizing constraint violations and minimizing task rewards.
    \item Maximizing constraint violations and maximizing task rewards. (maybe useful for training robustness?)
\end{enumerate}
The first one and third one seem more appropriate. But how to achieve this? We need to define the major goal and minor goal first.
If minimizing the constraint violation is the major objective, we have:

\begin{equation}
\begin{split}
  \max_{q} & \quad \E_{\rho_q}\Big[ \int q(a|s) Q_c^{\pi_{\theta_i}}(s,a) da \Big]\\
    s.t. & \quad \E_{\rho_q}\Big[\int q(a|s) Q_r^{\pi_{\theta_i}}(s,a) da \Big] \leq \epsilon_1 \\
    & \quad \E_{\rho_q}\Big[\KL(q(a|s)\Vert \pi_{\theta_i}) \Big] \leq \epsilon_2 \\
    & \quad \int q(a | s) da = 1, \quad \forall s \sim \rho_q
\end{split}
\end{equation}
This is something like a symmetrical form of CVPO. Another symmetrical form when the main objective is to reduce the reward is:

\begin{equation}
\begin{split}
  \max_{q} & \quad -\E_{\rho_q}\Big[ \int q(a|s) Q_r^{\pi_{\theta_i}}(s,a) da \Big]\\
    s.t. & \quad -\E_{\rho_q}\Big[\int q(a|s) Q_c^{\pi_{\theta_i}}(s,a) da \Big] \leq \epsilon_1 \\
    & \quad \E_{\rho_q}\Big[\KL(q(a|s)\Vert \pi_{\theta_i}) \Big] \leq \epsilon_2 \\
    & \quad \int q(a | s) da = 1, \quad \forall s \sim \rho_q
\end{split}
\end{equation}

By solving the convex optimization, we obtain the optimal adversarial distribution $\tilde{q}$ within the trust region of previous policy.

Then, how to solve the optimal adversarial state perturbation $\Delta S$? Unlike previous approaches that need to fix the agent policy and solve another MDP to predict $\Delta S$, we could use a parameter-free approach by directly optimizing it. In other words, we only need to solve the following optimization problem:

\begin{equation}
    \Delta S^* = \arg \min \E_{\rho_q} \left[ \KL(\pi (a | s+\Delta S) \Vert \tilde{q}(a | s)) \right], \quad s.t. \Delta S \in \Delta_\delta S
\end{equation}



Given each batch of data, we compute the optimal variational distribution $q^*$ as well as the adversarial distribution $\tilde{q}$, and we compute the optimal adversarial perturbations based on $\tilde{q}$. Then we aim to minimize the divergence between $\E_{\rho_q} \left[ \KL(\pi (a | s+\Delta S^*) \Vert q^*(a | s)) \right]$.

CVPO:
\begin{equation}
\begin{split}
   \max_{q} & \quad \E_{\rho_q}\Big[ \int q(a|s) Q_r^{\pi_{\theta_i}}(s,a) da \Big]\\
    s.t. & \quad \E_{\rho_q}\Big[\int q(a|s) Q_c^{\pi_{\theta_i}}(s,a) da \Big] \leq \epsilon_1 \\
    & \quad \E_{\rho_q}\Big[\KL(q(a|s)\Vert \pi_{\theta_i}) \Big] \leq \epsilon_2 \\
    & \quad \int q(a | s) da = 1, \quad \forall s \sim \rho_q
\end{split}
\end{equation}

M-step:
\begin{equation}
\begin{split}
    &\max_\theta \quad \E_{\rho_q}\Big[ \E_{q^*_i(\cdot|s)} \big[ \log \pi_\theta (a|s)\big]\Big] \\
    & s.t. \quad \E_{\rho_q}\big[ \KL(\pi_{\theta_i}(a|s)\Vert \pi_{\theta}(a|s)) \big] \leq \epsilon.
\end{split}
\label{eq:m_step_kl}
\end{equation}

Robust M-step:
\begin{equation}
\begin{split}
    \max_\theta  & \quad \E_{\rho_q}\Big[ \E_{q^*_i(\cdot|s)} \big[ \log \pi_\theta (a|s)\big]\Big] + \E_{\rho_q}\Big[ \E_{q^*_i(\cdot|s)} \big[ \log \pi_\theta (a|s+\delta_s^*)\big]\Big] \\
     s.t. & \quad \E_{\rho_q}\big[ \KL(\pi_{\theta_i}(a|s)\Vert \pi_{\theta}(a|s)) \big] \leq \epsilon  \\
    & \quad \E_{\rho_q}\big[ \KL(\pi_{\theta_i}(a|s)\Vert \pi_{\theta}(a|s+\delta_s^*)) \big] \leq \epsilon \\
    & \quad \delta_s^* = \arg\max_{\delta_s \in \Delta S} \E_{\tilde{a} \sim \pi(a|s+\delta_s)} \left[ Q_c(s, \tilde{a}) + \alpha Q_r(s, \tilde{a}) \right].
\end{split}
\label{eq:m_step_kl}
\end{equation}

Assume Lipschitz continuity of optimal policy $\TV(\pi^*(a|s)\Vert \pi^*(a|s+\delta_s)) \leq  K|\delta_s|$, then


% \begin{align}
%     \nabla_\theta \left(V_r^\pit(\mu_0) - \lambda V_c^\pit(\mu_0) \right) = \frac{1}{1-\gamma} \E_{s, a \sim \rho^\pi} \left[ \frac{\pit(a|\stt)}{\pi(a|s)} \nabla \pit(a|\stt) \left( Q^\pit_r(s,a) - \lambda Q^\pit_c(s,a) \right)\right]
% \end{align}

% Robust CMDP,

% \begin{equation}
% \begin{split}
%     \max_{\pi_\theta} \min_{\delta_r \in \Delta S} & \quad \E_{\rho_q}\Big[ \int \pi_\theta(a|s+\delta_r) Q_r(s,a)\Big]  \\
%      s.t.  \quad \max_{\delta_c \in \Delta S} & \E_{\rho_q}\big[ \int \pi_\theta(a|s+\delta_c) Q_c(s,a)\big] \leq \epsilon  \\
% \end{split}
% \end{equation}



% \begin{equation}
% \begin{split}
% V^\pi_f(\mu_0) = \frac{1}{1-\gamma} \underset{\substack{s \sim d^{\pi} \\ a \sim \pi \\ s' \sim P^{\pi}}} {\E}[f(s, a)] = \frac{1}{1-\gamma} \int\int  \rho^{\pi}(s, a) f(s,a) ds da, \quad f \in \{r, c\}
% \end{split}
% \end{equation}

% $
% V^\pi_r(\mu_0) = \frac{1}{1-\gamma} \E_{s, a \sim \rho^{\pi}}[r(s, a)] = \frac{1}{1-\gamma} \int\int  \rho^{\pi}(s, a) r(s,a) ds da
% $,
% $
% V^\pi_c(\mu_0) = \frac{1}{1-\gamma} \E_{s, a \sim \rho^{\pi}}[c(s, a)] = \frac{1}{1-\gamma} \int\int  \rho^{\pi}(s, a) c(s,a) ds da
% $.

% Then the safe RL objective can be written as an equivalent linear programming form:
% \begin{align}
%     \max_{\rho^\pi} \quad & \frac{1}{1-\gamma} \int\int  \rho^{\pi}(s, a) r(s,a) ds da \quad
%   s.t. & \frac{1}{1-\gamma} \int\int  \rho^{\pi}(s, a) c(s,a) ds da \leq \kappa 
%   %\\
% %   & \int \int \rho^{\pi}(s, a) c(s,a) ds da = 1
% \end{align}

% It is obvious that the agent without adversarial training is vulnerable, since the cost increases dramatically under adversarial attack. 
% The adversarial policy trained with random attacker is also not robust for the same reason. 
% The adversarial agents trained with MC or MR attacker are much more robust since the cost much is lower under adversarial attack. 
% Among most of the tasks, ADV-PPOL(MC) and ADV-PPOL(MR) achieves the lowest two cost under all the attackers. 
% On the other hand, under MC and MR attack, the cost of the converged adversarial policies still increases shows again the effectiveness of the attackers.


% \textbf{Evaluation of SA-PPOL.} 
% To evaluate the MAD attack that used in classic RL, we add another two baselines: SA-PPOL(MC) and SA-PPOL(MR). 
% Although the agents show some robustness against weak attackers such as AMAD, they suffer significantly under strong attackers such as MC and MR. 
% We also find that SA-PPOL(MC) and SA-PPOL(MR) are difficult to train. 
% They fail to converge for Ant-Run, Ant-Circle, and Drone-Run task. 
% The reason is that during training, the corrupted state will be more close to the true state that has lower reward. More details can be found in \todo{appendix}


%old abstract
% Safe reinforcement learning (RL) trains a policy to maximize the task reward while satisfying safety constraints. 
% Prior works indicate the vulnerability of trained deep RL policy by decreasing rewards under adversarial state perturbations. 
% This paper studies observational robustness in the safe RL setting, i.e., the constraint satisfaction performance of the trained policy under adversarial state perturbations. Both theoretical analysis and empirical results indicate that the optimal solutions of many safe RL problems are not robust against carefully designed attackers.
% We demonstrate the unique properties of designing effective adversarial attackers to increase the agent's constraint violation costs and propose two strong adversaries. One interesting and anti-intuitive finding is that a maximum reward attack can also induce unsafe behaviors for an optimal policy, and thus make the attack stealthy.
% We further show that baseline robust training techniques for classical RL tasks are ineffective in the safe RL setting.
% Therefore, we propose a much safer adversarial training algorithm and evaluate it in a wide range of safe RL tasks.
% We believe this is a pioneer work to establish the connection between robustness and safety regarding the constraint violations of RL.
